ForestFit : An R package for modeling tree diameter distributions

Modeling the diameter distribution of trees in forest stands is a common forestry task that supports key biologically and economically relevant management decisions. The choice of model used to represent the diameter distribution and how to estimate its parameters has received much attention in the forestry literature; however, accessible software that facilitates comprehensive comparison of the myriad modeling approaches is not available. To this end, we developed an R package called ForestFit that simplifies estimation of common probability distributions used to model tree diameter distributions, including the two- and three-parameter Weibull distributions, Johnson's SB distribution, Birnbaum-Saunders distribution, and finite mixture distributions. Frequentist and Bayesian techniques are provided for individual tree diameter data, as well as grouped data. Additional functionality facilitates fitting growth curves to height-diameter data. The package also provides a set of functions for computing probability distributions and simulating random realizations from common finite mixture models.

==> doc/tmp.tex <==
  \cormark[1]
  \fnmark[1]
  \ead{cvr_1@tug.org.in}
  \ead[url]{www.cvr.cc, www.tug.org.in}

  \credit{Conceptualization of this study, Methodology,
          Software}

  \address[1]{Indian \TeX{} Users Group, Trivandrum 695014,
       India}

  \author[2,4]{Han Theh Thanh}[style=chinese]

  \author[2,3]{T. Rishi Nair}[role=Co-ordinator,
                   suffix=Jr]
  \fnmark[2]
  \ead{rishi@sayahna.org}
  \ead[URL]{www.sayahna.org}

  \credit{Data curation, Writing - Original draft preparation}

  . . .
  . . .
  . . .
  \printcredits

